Dive Deeper Into Box for Object Detection

Anchor free methods have defined the new frontier in state-of-the-art object detection researches where accurate bounding box estimation is the key to the success of these methods. However, even the bounding box has the highest confidence score, it is still far from perfect at localization. To this end, we propose a box reorganization method(DDBNet), which can dive deeper into the box for more accurate localization. At the first step, drifted boxes are filtered out because the contents in these boxes are inconsistent with target semantics. Next, the selected boxes are broken into boundaries, and the well-aligned boundaries are searched and grouped into a sort of optimal boxes toward tightening instances more precisely. Experimental results show that our method is effective which leads to state-of-the-art performance for object detection.

==> ECCV20-AFOD-final/doc/abstract.tex <==
\begin{abstract}
%Bounding box is a conventional element in modern object detectors which is heavily relied while has not been fully exploited.In this paper, we present an anchor free detection model which break up the box to boundaries to facilitate the capability of model.A box decomposition and recombination (D\&R) strategy is proposed to optimize the learning in a bottom-up manner.Compared to the traditional detectors learn the task in an atomic style, D\&R unites the independent pixels in a bottom-up manner with negligible computation overhead and improve the quality of detection.A dynamic consistency strategy is approached in our model to align the candidate proposals and prediction scores together which guide network focus on the utile semantic elements.At inference stage, to make use of the boundary confidence scores learned during training, we improve the traditional NMS method by merging high quality boundaries into winner boxes. Experimental results show that the boundary level optimization with dynamic consistency for training and Box Merging NMS (BM-NMS) for inference outperforms current state-of-the-art one stage models.Without bells and whistles, we get 43.9\% in AP by using ResNeXt-64x4d-101-FPN as backbone under the setting of single-model and single scale testing on challenging COCO dataset. Compare to the RetinaNet, our model get 2.9\% in AP with the same backbone ResNet-101-FPN.
% Recently, anchor-free detectors are proposed to solve object detection in a per-pixel prediction fashion, analogue to semantic segmentation. Deeper research on the semantic and geometric properties of pixels is carried out in our paper, so that more accurate object detection can be achieved by reasoning from these dense pixels. Especially, a novel box decomposition and recombination (D\&R) method is proposed. We decompose object detection, an atomic task of estimating an independent bounding box of each instance, to a lower-level boundary prediction task. By analyzing which boundaries each pixel tends to model and summing up their geometric properties, a tight prediction of an instance is able to obtained. Moreover, an adaptive filtering method is presented to help our network fully benefit from semantic pixels while rule out distracting pixels inside an object bounding box, leading to an easy network convergence. Natively, our improvements including the D\&R method and the filtering method can be extended to a general detection framework without extra parameters. Experimental results show that equipped with these methods our detector outperforms current state-of-the-art one stage models.

% Anchor free methods have defined the new frontier in state-of-the-art object detection researches where accurate bounding box estimation is the key to the success of these methods. However, even with the bounding box with the highest confidence score, the sampled bounding boxes are still far from perfect. This motivates us to investigate a new method for bounding box reorganization given a set of bounding boxes from anchor free methods. Specifically, we propose a new and novel bounding box decomposition and recombination method which can consistently boost up the performance of \textcolor{red}{anchor free} object detection methods with a more accurate and tight bounding box that is derived from the given bounding boxes. Our method is based on boundaries re-ranking which is derived by our proposed IoU loss.  
% % After box merging NMS, we obtain a tight bounding box that are boundaries-aligned with the given boxes. 
% The proposed method is simple, fast, and is easily extended to a general detection framework with few parameters. Experimental results show that our method is effective which leads to state-of-the-art performance for one stage object detection. 

Anchor free methods have defined the new frontier in state-of-the-art object detection researches where accurate bounding box estimation is the key to the success of these methods. However, even the bounding box has the highest confidence score, it is still far from perfect at localization. 
To this end, we propose a box reorganization method (DDBNet), which can dive deeper into the box for  more accurate localization.
At the first step, drifted boxes are filtered out because the contents in these boxes are inconsistent with target semantics. Next, the selected boxes are broken into boundaries, and the well-aligned boundaries are searched and grouped into a sort of optimal boxes toward tightening instances more precisely.  
%This motivates us to investigate a box reorganization method (DDBNet), which can dive deeper into the box to strive for more accurate localization. Specifically, boxes are manipulated via a surgical operation named D\&R, which represents box decomposition and recombination toward tightening instances more precisely. %It should be noted that this D\&R operation is manipulated at the IoU loss.  
% The proposed method is simple, fast, and is easily extended to a general detection framework with few parameters. 
Experimental results show that our method is effective which leads to state-of-the-art performance for object detection.
\end{abstract}


==> ECCV20-AFOD-final/doc/conclusion.tex <==
\section{Conclusion}
  We propose an anchor-free detector DDBNet, which firstly proposes
  the concept of breaking boxes into boundaries for detection.
  The box decomposition and recombination optimizes the model training by uniting atomic pixels and updating in a bottom-up manner.
  We also re-evaluate the semantic inconsistency during training, 
  and provide an adaptive perspective to solve this problem universally with no predefined assumption. Finally, DDBNet achieves a state-of-the-art performance with inappreciable computation overhead for object detection.
  
  
  
  
  


==> ECCV20-AFOD-final/doc/experiments.tex <==
\section{Experiments}

\subsection{Experimental Setting}
\noindent\textbf{Dataset.} Our method is comprehensively evaluated on a challenging COCO detection benchmark\cite{lin2014microsoft}. 
Following the common practice of previous works\cite{OD-ICCV2019-FCOS,OD-ECCV2018-CornerNet,OD-ICCV2017-RetinaNet}, the COCO \textit{trainval35k} split (115K images) and the \textit{minival} split (5K images) are used for training  and validation respectively in our ablation studies. 
The overall performance of our detector is reported on the \textit{test-dev} split and is evaluated by the server. 
     
\noindent\textbf{Network Architecture.}
As shown in \Cref{figure: network-structure}, Feature Pyramid Network (FPN) \cite{OD-CVPR2017-FPN} is exploited as the fundamental detection network in our approach. The pyramid is constructed with the levels $P_{l}, l=3,4,...,7$  in this work. Note that each pyramid level has the same number of channels ($C$), where $C=256$. At the level $P_{l}$, the resolution of features is down-sampled by $2^{l}$ compared to the input size. 
Please refer to \cite{OD-CVPR2017-FPN} for more details. 
Note that four heads are attached to each layer of FPN. 
Apart from the regression and classification heads, a head for semantic consistency estimation is provided, consisting of a normal convolutional layer.
% Another head is designed for the boundary confidence prediction which contains a deformable convolutional layer and a normal convolutional layer. 
The regression targets of different layers are assigned in the same way as in \cite{OD-ICCV2019-FCOS}.
    
\noindent\textbf{Training Details.} Unless specified, all ablation studies take ResNet-50 as the backbone network. 
%  For the anchor free related settings, we choose \cite{OD-ICCV2019-FCOS} as our baseline.
To be specific, the stochastic gradient descent (SGD) optimizer is applied and our network is trained for 12 epochs over 4 GPUs with a  minibatch of 16 images (4 images per GPU). 
Weight decay and momentum are set as 0.0001 and 0.9 respectively.
The learning rate starts at 0.01 and reduces by the factor of 10 at the epoch of 8 and 11 respectively.
Note that the ImageNet pre-trained model is applied for the network initialization.  
%  The learning rate schedule follows the `$1\times$' setting as in MMDetection \cite{OD-arXiv2019-MMDetection}.
For newly added layers, we follow the same initialization method as in RetinaNet \cite{OD-ICCV2017-RetinaNet}. 
The input images are resized to the scale of $1333 \times 800$ as the common convention.
% The hyperparameter $\theta$ in \Cref{loss: bd-confidence-loss} determine the equality of predicted bounding boxes.  We experimentally set it as 0.9 in our paper.
For comparison with state-of-the-art detectors, we follow the setting in \cite{OD-ICCV2019-FCOS} that the shorter side of images in the range from 640 to 800 are randomly scaled and the training epochs are doubled to 24 with the same reduction at epoch 16 and 22.
% For other settings, we do not change.
     
\noindent\textbf{Inference Details.} 
At post-processing stage, the input size of images are the same as the one in training. 
The predictions with classification scores $s>0.05$ are selected for evaluation.
With the same backbone settings, the inference speed of DDBNet is same as the detector in FCOS\cite{OD-ICCV2019-FCOS}.
% The BM-NMS is applied with $N_t=0.5$ 
% and threshold $N_s$ is set to 0.95.



    % \cite{OD-ICCV2019-RepPoints} is new anchor free two stage model different from others,
            
        % \textbf{With or without B\&R in training}.
        %     \toupdate{update results}
        %     \begin{table}
        %     \caption{With or without B\&R in training}
        %         \label{tab:b&r-ablation}
        %             \begin{tabular}{c|c|cc|ccc}
        %             \toprule    
        %                                 & $AP$    & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
        %             \midrule
        %             None                & 33.6    & 53.1      & 35.0      & 19.8    & 38.1   & 43.7    \\ 
        %             B\&R                & 36.5    & 55.2      & 38.9      & 20.6    & 40.8   & 48.2         \\ 
        %             \bottomrule
        %         \end{tabular}
        %     \end{table}
  
%\label{subsubsection:ablation-study}            
%\subsubsection{Ablative experiments on proposed modules}

\subsection{Overall Performance}

 \begin{table*}[tb]
        \centering
        \caption{\textbf{Comparison with state-of-the-art two stage and one stage Detectors}
        (\textit{single-model and single-scale results}).
        DDBNet outperforms the anchor-based detector \cite{OD-ICCV2017-RetinaNet} by 2.9\% AP with the same backbone.
        Compared with anchor-free models, DDBNet is in on-par with these state-of-the-art detectors.
        $^\dag$ means the NMS threshold is 0.6 and others are 0.5.}
        \label{tab: sota}
        \resizebox{1.02\linewidth}{!}{
            \begin{tabular}{l|l|lll|lll}
                \toprule    
                Method            & Backbone  & $AP$    & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
                \midrule
                \textbf{Two-stage methods:} &&&&&&\\
                Faster R-CNN w/ FPN       \cite{OD-CVPR2017-FPN}          & ResNet-101-FPN                                     & 36.2 & 59.1 & 39.0 & 18.2 & 39.0 & 48.2 \\
                Faster R-CNN w/ TDM       \cite{OD-arXiv2016-Shrivastava} & Inception-ResNet-v2-TDM \cite{szegedy2017inception} & 36.8 & 57.7 & 39.2 & 16.2 & 39.8 & 52.1 \\ 
                Faster R-CNN by G-RMI     \cite{OD-CVPR2017-Huang}        & Inception-ResNet-v2                                 & 34.7 & 55.5 & 36.7 & 13.5 & 38.1 & 52.0 \\
                RPDet                     \cite{OD-ICCV2019-RepPoints}    & ResNet-101-DCN                                      & 42.8 & 65.0 & 46.3 & 24.9 & 46.2 & 54.7 \\
                Cascade R-CNN             \cite{OD-CVPR2018-Cai}          & ResNet-101                                          & 42.8 & 62.1 & 46.3 & 23.7 & 45.5 & 55.2 \\
                \midrule \midrule
                \textbf{One-stage methods:} &&&&&&\\               
                YOLOv2                    \cite{OD-CVPR2017-YOLO9000}     & DarkNet-19\cite{OD-CVPR2017-YOLO9000}               & 21.6 & 44.0 & 19.2 & 5.0  & 22.4 & 35.5 \\
                SSD                       \cite{OD-ECCV2016-Liu}          & ResNet-101                                          & 31.2 & 50.4 & 33.3 & 10.2 & 34.5 & 49.8 \\
                DSSD                      \cite{OD-arXiv2017-DSSD}        & ResNet-101                                          & 33.2 & 53.3 & 35.2 & 13.0 & 35.4 & 51.1 \\
                FSAF                      \cite{OD-CVPR2019-Zhucc}        & ResNet-101                                          & 40.9 & 61.5 & 44.0 & 24.0 & 44.2 & 51.3 \\
                RetinaNet                 \cite{OD-ICCV2017-RetinaNet}    & ResNet-101-FPN                                      & 39.1 & 59.1 & 42.3 & 21.8 & 42.7 & 53.9 \\
                CornerNet                 \cite{OD-ECCV2018-CornerNet}    & Hourglass-104                                       & 40.5 & 56.5 & 43.1 & 19.4 & 42.7 & 53.9 \\
                ExtremeNet                \cite{OD-CVPR2019-Zhou}         & Hourglass-104                                       & 40.1 & 55.3 & 43.2 & 20.3 & 43.2 & 53.1 \\
                FCOS$^\dag$               \cite{OD-ICCV2019-FCOS}         & ResNet-101-FPN                                      & 41.5 & 60.7 & 45.0 & 24.4 & 44.8 & 51.6 \\
                FCOS$^\dag$               \cite{OD-ICCV2019-FCOS}         & ResNeXt-64x4d-101-FPN                               & 43.2 & 62.8 & 46.6 & 26.5 & 46.2 & 53.3 \\
                FCOS$^\dag$ w/improvements\cite{OD-ICCV2019-FCOS}         & ResNeXt-64x4d-101-FPN                               & 44.7 & 64.1 & 48.4 & 27.6 & 47.5 & 55.6 \\
                \midrule
                DDBNet (Ours)                                         & ResNet-101-FPN          & 42.0 & 61.0 & 45.1 & 24.2 & 45.0 & 53.3 \\
                %DDBNet (Ours)$^\dag$                                  & ResNet-101-FPN          & 42.1 & 60.6 & 45.7 & 24.4 & 45.3 & 53.5 \\
                DDBNet (Ours)                                         & ResNeXt-64x4d-101-FPN   & 43.9 & 63.1 & 46.7 & 26.3 & 46.5 & 55.1 \\
                DDBNet (Ours)$^\mathsection$                          & ResNeXt-64x4d-101-FPN   & \textbf{45.5} & \textbf{64.5} & \textbf{48.5} & \textbf{27.8} & \textbf{47.7} & \textbf{57.1} \\
                \bottomrule
            \end{tabular}
        }
        \scriptsize{
            \begin{flushleft}
                $^\mathsection$ GIoU\cite{Rezatofighi_2018_CVPR} and Normalization methods of `improvements' proposed in FCOS\cite{OD-ICCV2019-FCOS} are applied, ctr.sampling in `improvements'\cite{OD-ICCV2019-FCOS} are not compatible with our setting and we do not use.
            \end{flushleft}
        }
        \vspace{-.4in}
    \end{table*}

% The shorter side of images in the range from 640 to 800 are randomly scaled during the training and the training epoches are doubled to 24 epoches with `$2\times$' learning rate schedule settings \cite{OD-arXiv2019-MMDetection}.
We compare our model denoted as DDBNet with other state-of-the-art object detectors on the \textit{test-dev} split of COCO benchmark, as listed in \Cref{tab: sota}.
    % For other settings, we do not change.
Compared to the anchor-based detectors, our DDBNet shows its competitive detection capabilities. Especially, it outperforms RetinaNet\cite{OD-ICCV2017-RetinaNet} by 2.9\% AP. When it comes to the anchor-free detectors, especially detectors such as FCOS\cite{OD-ICCV2019-FCOS} and CornerNet\cite{OD-ECCV2018-CornerNet} benefiting from the point-based representations, our DDBNet achieves performances gains of 0.5\% AP and 1.5\% AP respectively.
Based on the ResNeXt-64x4d-101-FPN backbone \cite{SPEED-CVPR2017-ResNeXt},
DDBNet works better than \cite{OD-ICCV2019-FCOS} with a 0.7\% AP gain.
Especially for large objects, our DDBNet gets 55.1\% AP, better than 53.3 \% reported in FCOS\cite{OD-ICCV2019-FCOS}.
% Note that, FCOS sets the NMS threshold to 0.6 instead of 0.5, which is different from the conventional setttings in other works. 
%Our DDBNet provides stable results under the two settings in all AP metrics. Thus, we report the results following the conventional settings. 
We also apply part of 'improvement' methods proposed in FCOS to DDBNet and gets 0.8\% better than the FCOS with all `improvements' applied.
To sum up, compared to detectors exploiting point-based representations, our DDBNet can similarly benefit from the mid-level boundary representations without heavy computation burdens. Furthermore, DDBNet is compared to several two stage models. It overpasses \cite{OD-CVPR2017-FPN} by a large margin.

\vspace{-.1in}
\subsection{Ablation Study}

In this section, we explore the effectiveness of our
method, including two main modules of box D\&R module and semantic consistency module. Additionally, we conduct in-depth analysis of the performance metrics of our method.

\subsubsection{Comparison with Baseline Detector}\mbox{}

It should be noted that FCOS detector\cite{OD-ICCV2019-FCOS} without the centerness branch in both training and inference stages is taken as our baseline. 
Here we conduct in-depth analysis of the performance metrics of our method. 
% More qualitative experiments are provided in supplementary material.

\noindent\textbf{Box D\&R module.} 
As shown in \Cref{tab:b&r-ablation}, by incorporating the D\&R module into the baseline detector, a 1.2\% $AP$ gain is obtained, which proves that our D\&R module can boost the overall performance of the detector. Especially for the $AP_{75}$, a 1.4\% improvement is achieved, which means that D\&R performs better on localization even in a strict IOU threshold. Furthermore, D\&R module achieves a better performance on large instances according to the large gain on $AP_L$. 
With explicit boundary analysis, large instances are often surrounded by numbers of predicted boxes. As a result, it gets easier to find the well-aligned boundaries, then the boxes re-organization can be more effective.  
%Compared to the baseline results of 53.1\%, 35.0\%, 18.9\% and 38.2\% in metrics including $AP_{50}$, $AP_{75}$, $AP_{S}$ and $AP_{M}$, D\&R obtains stable performance gains of 0.9\%, 1.4\%, 0.8\% and 0.8\% respectively, which shows the stability of our proposed module.
Compared to the baseline results in metrics including $AP_{50}$, $AP_{S}$ and $AP_{M}$, D\&R obtains stable performance gains respectively, which shows the stability of our proposed module.
By breaking the atomic boxes into boundaries, D\&R module makes each boundary find the better optimization direction. The optimization of boundary is not limited by the box its in, instead of depending on a sorted of related boxes. Generally, by adjusting the boundary optimization, the detection network is learnt better.  
            % This module can also transfer to other anchor free module fo
    \begin{table*}[t]
        \centering
        \caption{\textbf{Ablative experiments for DDBNet on the COCO \textit{minival} split.} We evaluate the improvements brought by the Box Decomposition and Recombination(D\&R) module and the semantic consistency module.}
        \resizebox{.68\linewidth}{!}{
            \begin{tabular}{ccc|l|ll|lll}
                \toprule    
                \multicolumn{3}{c|}{ Modules }    & $AP$    & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
                Baseline & D\&R & Consistency     &  & & & & & \\
                \midrule
                \checkmark &            &            & 33.6          & 53.1          & 35.0          & 18.9          & 38.2          & 43.7  \\ 
                \checkmark & \checkmark &            & 34.8          & 54.0          & 36.4          & 19.7          & 39.0          & 44.9  \\
                \checkmark &            & \checkmark & 37.2          & 55.4          & 39.5          & 21.0          & 41.7          & 48.6  \\ 
                \checkmark & \checkmark & \checkmark & \textbf{38.0} & \textbf{56.5} & \textbf{40.8} & \textbf{21.6} & \textbf{42.4} & \textbf{50.4}  \\
                \bottomrule
            \end{tabular}
        }
        \label{tab:b&r-ablation}
    \end{table*}        
    

    
\noindent\textbf{Semantic Consistency module.}
The semantic consistent module described in \Cref{subsec:reg-cls-consist} presents an adaptive filtering method. It forces our detection network into autonomously focusing on positive pixels whose semantics are consistent with the target instance. As shown in \Cref{tab:b&r-ablation}, the semantic consistency module contributes to a significant performance gain of 3.6\% $AP$ compared to the baseline detector. This variant surpasses the baseline by large margins in all metrics. 
Due to that the coarse bounding boxes would contain backgrounds and distractors inevitably, the network is learnt with less confusion about the targets when equips our adaptive filtering module. More ablation analysis on semantic consistency module is provided in \Cref{subsubsec:ana-sc}.
        
\noindent\textbf{Cooperation makes better.}
In our final model denoted as DDBNet, the semantic consistency module first filters out a labeling space of pixels inside each instance that is strongly relative to the geometric and semantic characteristics of the instance. The box predictions of the filtered positive pixels are further optimized by the D\&R module, leading to more accurate detection results. Consequently, DDBNet achieves 38\% AP, better than all the variants in \Cref{tab:b&r-ablation}. Our method boosts detection performance over the baseline by 2.7\%, 4.2\%, and 6.7\% respectively on $AP_S$, $AP_M$, $AP_L$.
%With a well defined learning space, 
%the D\&R strategy performs better on the baseline model.
%We get 38\% AP performance in the final model.
%From the aspect of sizes, the final model gets 4.2\% and 6.7\% improvements on middle and large instances respectively and increasing on small objects is 2.7\% compare to the baseline model.


\subsubsection{Analysis on D\&R Module.}\mbox{}

\noindent\textbf{Statistical comparison with conventional IoU Loss.}
As we mentioned in \Cref{subsec:box-decom-recom}, IoU loss with D\&R updates the gradient according to the optimal boundary scores.
To confirm the stability of D\&R module, we plot the average IoU scores and variances of boxes before and after D\&R respectively. 
We can see that with D\&R module, the average values of IoU scores are higher than the means of origin IoU scores by a large margin around 10\% in the whole training schedule, as in \Cref{figure: mean-iou-compare}. 
At the start of training, the mean of optimal boxes gets 0.47  which is better than 0.34 of origin boxes. 
As training goes on, both average scores of origin and optimal boxes increase and remain at 0.77 and 0.86 at the end.
Variances of IoU scores with D\&R are much lower than the origin IoU scores, which indicates D\&R module improves the overall quality of boxes and provides better guidance for training.
% The runtime is measured on a single TITAN XP GPU.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\linewidth]{figure/dr-compare-appendix.pdf} 
%     \caption{Average IoU scores for all predicted boxes during the training.
%     Red line denotes the IoU scores with D\&R module and the blue line is the IoU scores without optimization.
%     Vertical lines indicate the variance of IoU scores.}
%     \label{figure: mean-iou-compare}
% \end{figure} 




\iffalse








\fi
\begin{figure}[tb!]
    \centering
    \pgfplotsset{
        width =0.58\linewidth,
        height=0.36\linewidth
    }
\begin{tikzpicture}[scale=1]
\begin{axis}[minor tick num=0,
xmin=-0.5, xmax=12,
ymin=0.25, ymax=0.95,
mark size=1.0pt,
%ymax=5000,
%xtick={0.3,0.4,...,0.8},
ytick={0.3,0.5,...,0.9},
%yticklabel style={/pgf/number format/.cd, fixed, fixed zerofill, precision=1, /tikz/.cd},
%scaled y ticks=base 10:0, 
xlabel={epoch},
ylabel={IoU},%{$|\vec{w}^{(t+1)}-\vec{w}^{(t)}|$}, 
xlabel near ticks,
ylabel near ticks,
legend style={
  draw=none,
  at={(1.0,.28)},
  anchor=west,
  legend columns=1},
]
\addplot [color=red, only marks, mark=o, line width=1.0pt]
    plot [error bars/.cd, y dir = both, y explicit]
    table [x={iter},  y={dr-mean}, y error={var}]  {dr-iou.mat};
\addplot [color=blue, only marks, mark=o, line width=1.0pt]
    plot [error bars/.cd, y dir = both, y explicit]
    table [x={iter},  y={iou-mean}, y error={var}]     {origin-iou.mat};
\legend{IoU w/~D\&R, IoU w/o~D\&R}
\end{axis}
\end{tikzpicture}
\caption{\textbf{Average IoU scores for all predicted boxes during the training.}
    The red points denote the IoU scores with D\&R module while the blue points are the IoU scores without optimization.
    Vertical lines indicate the variance of IoU scores.}
    \label{figure: mean-iou-compare}

\end{figure}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.88\linewidth]{figure/dr-appendix-visualize.pdf} 
    \caption{
        \textbf{Illustration of improved box predictions provided by our DDBNet.}
        We visualize the boxes before the decomposition (left images of the pairs) and the boxes after the recombination (right images of the pairs). \textbf{Red}: ground-truth boxes. \textbf{Green}: the predictions, where the lighter colors indicate higher IoU scores. \textbf{Black}: the boxes with low score, which will be masked according to the regression loss.
        Boxes ranked by D\&R module are much better organized than the origin boxes and the localizations are much correlated to the instances.
        % Boxes with low IoU scores contribute to better localization for training.
        All the results are from DDBNet with ResNet-50 as backbone on $trainval35k$ split.}
    \label{figure: dr-appendix-visualize}
\end{figure*} 

\noindent\textbf{Visualization on D\&R module.} 
We provide some qualitative results of box predictions before and after incorporating the D\&R module into the baseline detector, 
as shown in \Cref{figure: dr-appendix-visualize}.
For clear visualization, we plot origin boxes and boxes after recombination individually. Predictions are presented in green and the lighter colors indicate higher IoU scores.
% Boxes without D\&R are learned in an atomic manner which provide a non-ideal prediction during the training.
With D\&R module, boundaries are recombined together to obtain a tighter box of each instance.
The distribution of boxes after D\&R module is fitter than the origin boxes which is robust than the conventional regression.
As we mentioned in \Cref{subsec:box-decom-recom}, there exists recombined low-rank boxes with boundary scores lower than the origin.
These boundaries are masked according to the \Cref{loss: our-iou}.

\label{subsubsec:ana-sc}
\subsubsection{Analysis on Semantic Consistency}\mbox{}

            \begin{table}[tb!]
                \centering
                \caption{\textbf{Comparison among different positive assignment strategies.} 
                `None' means no sampling method is applied.
                `PN' denotes as the definition in \cite{OD-arXiv2019-FoveaBox}, 
                 which means center regions are positive and others are negative. 
                `PNI' is the sampling used in \cite{OD-CVPR2019-Zhucc,OD-CVPR2019-Wang},
                ignore regions are added between positive and negative.
                Note that the consistency term is not included in this table.}
                \begin{tabular}{c|l|ll|lll}
                    \toprule    
                    Settings   & $AP$    & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
                    \midrule
                    None        & 33.6     & 53.1    & 35.0    & 18.9     & 38.2    & 43.7  \\ 
                    PN        & 34.2     & 53.2    & 36.3    & 20.8     & 38.9    & 44.2  \\
                    PNI       & 33.7     & 53.0    & 35.5    & 17.9     & 38.3    & 44.1  \\
                    Ours      & \textbf{35.3}     & \textbf{55.4}    & \textbf{37.1}    & \textbf{20.9}     & \textbf{39.6}    & \textbf{45.9}  \\ 
                    \bottomrule
                \end{tabular}
                \label{tab:consistency-ablation}
            \end{table}
\noindent\textbf{Dynamic or predefined positive assignment.} 
To further show the superiority of dynamic positive assignment in semantic consistency module, we investigate other variants using different predefined strategies mentioned in previous works. FoveaBox\cite{OD-arXiv2019-FoveaBox} (denoted as `PN') applies center sampling in their experiments to improve the detection performance. 
This center sampling method defines the central area of a target box based on a constant ratio as positive while the others as negative.
% FSAF\cite{OD-CVPR2019-Zhucc} and GA-RPN\cite{OD-CVPR2019-Wang} 
`PNI' is taken used in \cite{OD-CVPR2019-Zhucc, OD-CVPR2019-Wang} which exploits positive, ignore and negative regions for supervised network training.
According to the result in \Cref{tab:consistency-ablation},
`PN' (second line) gets slight improvement compared to the baseline where no sampling method is adopted. 
So restricting the searching space to the central area makes sense in certain cases and indeed helps improve object detection.
But the 'PNI' gets a lower performance, especially on $AP_S$. Namely, adding an ignore region between the ring of negative areas and the central positive areas does not further improve the performance and gets a large drop on the detection of small objects.
The limited number of candidates of small objects and the lower ratio of positive candidates in `PNI' result in the poor detection capability.
Contrastively, our proposed filtering method does not need to pre-define the spatial constraint while show best performances in all metrics.

\begin{table}[tb!]
    \centering
    \caption{\textbf{Comparison among different ratio settings.} 
    where $c$ is the sampling ration for each instance.}
    \begin{tabular}{c|l|ll|lll}
        \toprule    
        ratios   & $AP$    & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
        \midrule
        $c=0.4$                    & 34.6 & 54.2 & 36.6 & 19.1 & 38.5 & 45.2  \\
        $c=0.5$                    & 34.1 & 53.5 & 35.9 & 19.2 & 38.4 & 44.2  \\ 
        $c=0.6$                    & 34.7 & 54.2 & 36.5 & 19.0 & 38.7 & 45.5  \\ 
        $c=0.7$                    & 35.1 & 54.6 & \textbf{37.1} & 19.3 & 39.1 & 45.7  \\ 
        $mean$                     & \textbf{35.3}     & \textbf{55.4}    & \textbf{37.1}    & \textbf{20.9}     & \textbf{39.6}    & \textbf{45.9}  \\ 
        \bottomrule
    \end{tabular}
    \label{tab:consistency-ratio}
\end{table}
\noindent\textbf{Adaptive or constant ratio.} 
%Another reason why our semantic consistency module performs stably on objects of all sizes lies in the dynamic ratio $mean$ in \Cref{semanticeq}.
As mentioned in \cref{subsec:reg-cls-consist}, we investigate the constant ratio to replace the adaptive selection by mean. Four variants are obtained where the constant ratio is set from 0.4 to 0.7. 
%We compare the initial variant using the standard semantic consistency module with the mean threshold with the four variants, 
For instance $I$ with $M$ candidates, top $\left \lfloor c \times M \right \rfloor$  candidates are considered as positive, and others are negative, where $c$ is the constant sampling ratio applied to all instances. 
As shown in \Cref{tab:consistency-ratio}, these results indicate that the adaptive way in our method is better than the fixed way to select positives from candidates.

%performances of four variants are not linearly relative to the number of samples, which indicates that using constant ratios to define learning spaces of objects with different sizes is not the best choice.
%The dynamic ratio $mean$ takes this issue into account and gets best results among all metrics.
            % partially it is due to that the scenario of \cite{OD-CVPR2019-Zhucc,OD-CVPR2019-Wang} is different from this work.
            % \todo{visualize result}
%To compatible with \Cref{semanticeq} in training, we choose a high threshold $N_s$ at inference, only the boxes with lower scores which highly coincident with the box with top score are take into consideration.
%According to the experiments, we find out that merging boxes slightly inferior with the best predicted box can get better quality.
%The performance of BM-NMS in all metrics is more robust than the traditional NMS with negligible deceleration. 
%BM-NMS benefits from the high quality predicted boxes but ignored in traditional NMS. 
% The runtime is measured on a single TITAN Xp GPU.
%Different from the scenario of \cite{OD-CVPR2019-He} learning localization variance during training, the inherent ambiguities of annotation is not considered in our work.










==> ECCV20-AFOD-final/doc/intro.tex <==
\section{Introduction}

% Convolutional neural network (CNN) is one of the most representative model of deep learning which widely used in computer vision.
%Thanks to the expressive capability of CNN, the opportunity of joint optimization of related tasks becomes feasible.
%CNN based object detection combines classification and bounding box regression into a multi-task style and got remarkable improvement in recent years. 
% Mainstream of object detection models can be categorized into two types. 
% One is anchor based, which includes one stage models and two stage models, 
% one stage based frameworks focus on the requirement of efficiency and two stage model explored on high quality. 
% The other is anchor free based, anchor free based methods aim to get rid of preassigned anchors, 
% which provide a new perspective on model designs and got great improvement recently.
% Number of design parameters is significantly reduced.
% Anchor free based methods follow the anchor based design rule on feature extraction and learning target.
% These kind of approaches have following features during training and inference.

%At training stage, convolution kernels slide on feature maps in traverse manner, regression and classification targets are learned locally.
%For inference, pixels of same categories are chosen and clustered according to the Intersection over Union (IoU) scores, 
%the most confidential pixel is regarded as the final result for an instance.
%It is reasonable to consider pixels in feature maps responsible for the representation of locations and categories they belong to, as using pixel to present objects is efficient for training and inference in deep learning frame.
%While  \textit{pixel presents objects} design style has following limitations may overlooked: 
%\begin{itemize}
%    \item \textbf{Features are learned locally.} 
%    The capability of the model is constrained by the receptive fields,
%    which means the global information is hard to capture by the small convolution kernels.
%    \item \textbf{Winner pixel takes all.} 
%    Only pixel with highest score is picked up at post processing stage for each instance, rest of boxes which have higher boundary qualities are not used after clustering.
%\end{itemize}
%We hope we can take use of instance-wise features for a better feature learning.
%While to learn features in global, 
%how to determine the effective learning space and learn instance-wise features efficiently are critical problems, which due to following issues
%\begin{itemize}
%    \item \textbf{Annotation inconsistency.} 
%    The annotation of bounding box for each instance is not consistent to the corresponding target. 
%    We know that to present an object with a box is straight forward for annotation and robust for regression,
%    while how to judge whether pixel in boxes has positive or negative effects for this multi task is still undetermined. 
%    \item \textbf{More capacity, less efficiency.}
%    Emperically, more deeper convolution network can bring better performance.
%    While trying to get further improvement on accuracy in this way %sacrifice on speed.
%\end{itemize}
    

% For example, an instance at a feature level with $20 \times 20$ size, only 9 neighbor pixels in previous layers are learned with a $3 \times 3$ kernel and only one pixel present the instance location and category after the post processing.
% The instance wise features are ignored during the training due to the property of CNN. 
% As most features are learned locally, instance wise features are not taken used at inference.
%According to these observations, it is nature to raise a question:
%Can we make use of instance wise features to improve the precision with no pain on efficiency and keep consistency in object detection framework?

%To answer this question, we present a novel anchor free model which take advantage of instance wise features in training and inference to enhance the training procedure and post processing.
%A box decomposition and recombination strategy is applied to optimize the network training. 
%We decompose boxes into boundaries and recombine boundaries as optimized boxes.
%The optimized boxes improve the gradient of regression and relax the receptive field from local to global without further computation during training.
%A general concept of box decomposition and recombination is shown in \Cref{figure:D_R-visualize}. 
%With the decomposed boxes, the distribution of boundaries confidence for instances are learned during the training and couple with traditional non-maximum suppression at inference stage, 
%which further improve the prediction result with features of instances fully used.
%Detail of Box Merging Non-Maximum Suppression (BM-NMS) is described in \Cref{subsec:bm-nms}

%Due to the inconsistency between mask of instance and bounding boxes,
% figure here
%we find out that taking all pixels of instance into account may abused and cause unstable on box decomposition and recombination. 
%Many previous anchor free based works \cite{OD-arXiv2019-FoveaBox,OD-ICCV2019-FCOS,OD-CVPR2019-Wang} presented solutions on solving this problem by finding an optimal learning space.
%A soft threshold called centerness is used in \cite{OD-ICCV2019-FCOS}. 
%\cite{OD-CVPR2019-Wang} assigns groundtruth instances to different feature levels with an expectation that placing more anchors around object's center.
%In short, a predefined center field is needed in these approaches. 
%These methods assume that the center area is the most related part to an instance and other parts have low confidence and cause negative effects for model learning.
%It is reasonable to degrade the importance of features close to boundaries, but the predefined center field may not cover all cases in real world, examples show in \Cref{figure:inconsistency-example}. 

%Whether the center features can present various kinds of instances are still an outstanding issue.
% \todo{example}
%Here we apply a regression and classification consistency strategy in training which provide a new aspect on solving this problem.
%A simple dynamic filtering strategy is used to guide the network focus on the high confidence part and reject the low confidence features during the training.
%Since there is no spatial constraint in our method, no hyper-parameters are needed.
%The detail description is shown in \Cref{subsec:reg-cls-consist}.

%The main contribution of this work lies in following aspects.
%(1) We propose a new anchor free model which take use of instance wise features with negligible computation overhead.
%To our best knowledge, the idea of breaking boxes into boundaries for training and inference are first integrated proposed in this task.
%(2) We rethink the inconsistency between annotation and learning targets from a new point of view in this paper,
%an universal consistency strategy is proposed to this problem.
%(3) \todo{mention final result here.}

%Contribution summary

%%%%%add by davina
Object detection is an important task in computer vision, which requires predicting a bounding box of an object with a category label for each instance in an image. 
State-of-the-art techniques can be divided into either anchor-based methods \cite{OD-CVPR2014-RCNN,OD-ICCV2015-FastRCNN,OD-TPAMI2017-FasterRCNN,OD-arXiv2017-DSSD,OD-ECCV2016-Liu,OD-CVPR2018-Cai,he2017mask,OD-CVPR2017-YOLO9000,redmon2018yolov3}
and anchor-free methods \cite{OD-CVPR2016-YOLO, OD-ICCV2019-FCOS, OD-ICCV2019-CenterNet, OD-CVPR2019-Zhou, OD-ICCV2019-RepPoints, jie2016scale}. 
Recently, the anchor-free methods have increasing popularity over the anchor-based methods in many applications and benchmarks\cite{lin2014microsoft, everingham2015pascal, deng2009imagenet, OD-CVPR2012-Geiger}.
%In a nutshell, anchor-free methods offer the following advantages over the anchor-based methods: 
%1) It has significantly less number of parameters brought by predefined anchors;
%2) It is computationally faster in both training and testing;
%3) It alleviates the adverse effects caused by a large number of false candidates in the background which implicitly resolve the imbalance problem between positive and negative samples.
Despite the success of anchor-free methods, 
one should note that these methods still have limitations on their accuracy, which are bounded by the way that the bounding boxes are learned in an atomic fashion. %defined and obtained by a naive NMS method. 
Here, we discuss two concerns of existing anchor-free methods which lead to the inaccurate detection.

%which motivate us to propose our bounding box decomposition and recombination method:
% \begin{itemize}
    % \item 
    
    
    % \noindent\textbf{Winner pixel takes all.}
    \iffalse{
    \noindent\textbf{Local wise regression is limited.}
    In general, anchor-free methods estimate a bounding box at each position of the feature map that is obtained from the last layer of the backbone network.
    For simplicity, we denote each position of a feature map as a pixel in this paper.
    As shown in \Cref{figure:D_R-visualize}, 
    the dotted box and corresponding pixel are presented in the same color.
    Limited by the receptive fields of convolution kernels, boxes learned in an atomic way have potential defects on precision.
    % only the pixel with the highest detection score is selected to predict the bounding box of an object at the post processing stage.
    % This strategy is sometimes aggressive and inefficient.
    Four boundaries of a box may not be well aligned to the ground truth simultaneously.%,  as shown in \Cref{figure:D_R-visualize}.}
    % Not only because the four boundaries of a box may not be well aligned to the ground truth simultaneously,
    % but also the less confident boxes that potentially have higher boundary qualities will be discarded after the Non-Maximum Suppression (NMS) \cite{rosenfeld1971edge} as shown in \Cref{figure:D_R-visualize}.
    Thus, the accuracy of an anchor-free detector is bounded by the quality of the boxes defined at each pixel in the last layer feature map, where the last layer feature map is usually at a lower resolution than the original input image as demonstrated in many representative backbone networks.

    % \item 
    \noindent\textbf{The predefined importance of each pixel is inconsistent with the semantics.} 
    Without any prior knowledge about an object, 
    pixels in an object bounding box usually show uniform-distributed or gaussian-distributed effects in the learning stage of the anchor-free detectors such as the FCOS \cite{OD-ICCV2019-FCOS} and the CornerNet \cite{OD-ECCV2018-CornerNet} detectors. 
    However, it is inevitable to include pixels from background in the bounding box, and these background regions are not uniformly distributed, as illustrated in \Cref{figure:inconsistency-example}. 
    Thus, taking all predefined pixels as positive targets in the training stage would lead to a significant semantic inconsistency, which hampers the accuracy of the predicted boxes from the network.
    }\fi
    
    % \item 
    %First, the predefined center key-point is inconsistent with the semantics.
    %As all we known that center key-point is essential for anchor-free detectors. It is a common strategy to %predefined positive center key-point inside an object's bounding box as a Uniform or Gaussian %distribution in the training stage of the anchor-free detectors such as FCOS \cite{OD-ICCV2019-FCOS} and %CornerNet \cite{OD-ECCV2018-CornerNet}. 
    %However, it is inevitable to pull in noisy pixels from background to positives, as illustrated in %\Cref{figure:inconsistency-example}.
    %Thus, taking the predefined trivial strategy to define positive target would lead to a significant %semantic inconsistency, which hampers the accuracy of the predicted boxes from the network. 
    
    First, the definition of center key-points \cite{OD-ICCV2019-CenterNet} is inconsistent with their semantics.
    As we all know that center key-point is essential for anchor-free detectors. It is a common strategy to embed positive center key-points inside an object bounding box into a Uniform or Gaussian distribution in the training stage of the anchor-free detectors such as FCOS \cite{OD-ICCV2019-FCOS} and CornerNet \cite{OD-ECCV2018-CornerNet}. 
    However, it is inevitable to falsely consider noisy pixels from background as positives, as illustrated in \Cref{figure:inconsistency-example}.
    Namely, exploiting a trivial strategy to define positive targets would lead to a significant semantic inconsistency, degrading the regression accuracy of detectors.  
    
    %Second, local wise regression is limited.
    %%Generally, each center key-point is responsible to produce a corresponding atomic prediction box through a local wise regression.
    %Limited by the receptive fields of convolution kernels, the atomic predicted boxes has potential defects on precision.
    %As shown in \Cref{figure:D_R-visualize}, the dotted predicted box and corresponding center key-point are presented in the same color.
    %Although each predicted box is surrounding the object, it is imperfect that four boundaries are not well aligned to the ground truth simultaneously.
    %As a result that choosing a high score box at inference stage as the final detection result is sometimes defective.
    %The accuracy of anchor-free detectors is bounded by regarding the predicted boxes as atoms.
    
    Second, local wise regression is limited. Concretely, a center key-point usually provides box predictions in a regional/local-wise manner, which potentially defects the detection accuracy. The local-wise prediction results from the limitation of the receptive fields of convolution kernels, and the design of treating each box prediction from each center key-point as an atomic operation. 
    As shown in \Cref{figure:D_R-visualize}, the dotted predicted box and corresponding center key-point are presented in the same color.
    Although each predicted box is surrounding the object, it is imperfect because four boundaries are not well aligned to the ground truth simultaneously.
    As a result, choosing a box of high score at inference stage as the final detection result is sometimes inferior.
% \end{itemize}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.7\linewidth]{inconsistency-example} 
    \caption{\textbf{An illustration of the inconsistency between the semantics of center key-points inside a bounding box and their annotations.} Pixels of backgrounds in the red central area are considered as positive center key-points, which is incorrect.}
    \label{figure:inconsistency-example}
\end{figure} 

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.66\linewidth]{D_R-visualize} 
    \caption{\textbf{An illustration of the boundary drifts in box predictions of general anchor-free detectors.} Limited by regional receptive fields and the design of treating each box prediction as an atomic operation in general detectors, each predicted box with dotted line is imperfect where four boundaries are not well aligned to the ground truth simultaneously. After box decomposition and combination, the reorganized box with red color gets better localization.}
    \label{figure:D_R-visualize}
\end{figure} 

% Considering the above two issues, to make the best use of the model capability of the dense prediction network, careful studies on the functional rule of pixels in both training and inference stages should be carried out.

%To tackle the inaccurate detection problem, we present a novel bounding box reorganization method which consists of box decomposition, boundaries ranking, and box recombination after a pre-operator of semantic consistency filter.

%To tackle the inaccurate detection problem, we present a novel bounding box reorganization method to reproduce more accurate target box for box regression.
%Specifically, at the first step, the corresponding box predictions of central pixels inside an instance are first collected to form a coarse distribution of the instance.
%Then, these boxes are decomposed into four sets of boundaries to model an instance at a lower refined level, where the confidence of each boundary is evaluated according to the IoU.
%Next, these boundaries are sorted and recombined to form a sort of more accurate boxes for each object.
%Finally, the reorganization accurate boxes are taken as the target of box regression.
%Meanwhile, a semantic consistency module is proposed to rule out noisy center pixels from the background that allows our method to focus on pixels that are strongly related to the target instance semantically.
%Thus, box predictions from these semantic csonsistent pixels can form a more tight and robust distribution of the instance, which leads to better performance for box decomposition and recombination.
%Our semantic consistency module is an adaptive strategy without extra hyper-parameters for predefined spatial constraints, which totally beats the predefined center key-point predefined strategy.

To tackle the inaccurate detection problem, we present a novel bounding box reorganization method, which dives deeper into box regressions of center key-points and takes care of semantic consistencies of center key-points.
This reorganization method contains two modules, denoted as box decomposition and recombination (D\&R) module and semantic consistency module.
Specifically, box predictions of center key-points inside an instance form an initial coarse distribution of the instance localization. This distribution is not well aligned to the ideal instance localization, and boundary drifts usually occur. 
The D\&R module is proposed to firstly decompose these box predictions into four sets of boundaries to model an instance localization  at a lower refined level, where the confidence of each boundary is evaluated according to the deviation with ground-truth. 
Next, these boundaries are sorted and recombined to form a sort of more accurate box predictions for each instance, as described in \Cref{figure:D_R-visualize}.
Then, these refined box predictions contribute to the final evaluation of box regressions.

Meanwhile, the semantic consistency module is proposed to rule out noisy center key-points coming from the background, which allows our method to focus on key-points that are strongly related to the target instance semantically.
Thus, box predictions from these semantic consistent key-points can form a more tight and robust distribution of the instance localization, which further boosts the performance of the D\&R module.
Our semantic consistency module is an adaptive strategy without extra hyper-parameters for predefined spatial constraints, which is superior to existing predefined strategies in \cite{OD-CVPR2019-Zhucc, OD-CVPR2019-Wang, OD-ICCV2019-FCOS}.



%\todo{Unlike the traditional detection methods, regarding detection as an atomic task that independently estimates each bounding box, we dive much deeper into the characteristic of the dense prediction of pixels, and break up bounding box predictions into underlying boundary-related operations. After analyzing different effects brought by each pixel to the boundaries, more accurate box predictions are deduced from these dense pixels. Meanwhile,a dynamic filtering strategy is proposed to guide the network focus on useful semantic pixels inside each instance rather than backgrounds or distractors during the training stage. Thus, high semantic consistency between the pixel prediction and the target instance is achieved, so that candidate proposals with high scores usually align with an instance tightly. Since there is no spatial constraint predefined in our method, no hyper-parameters are needed.}  

%Especially, a box decomposition and recombination method is proposed to   make predicted bounding box aligned more accurately with an instance. In the literature, a detector simply select a candidate box with the highest detection score as an instance prediction via NMS. In contrast, we decompose each candidate bounding box into four boundaries, and then a ranking strategy is exploited to sort boundaries of all the candidate boxes by the boundary accuracy, and finally accurate box prediction is generated by the four boundaries which rank first respectively. The box decomposition and recombination method is exploited in both training and inference stages, and makes full use of pixels with different attributes. Namely, different pixels contribute better to different boundary predictions. 

%Secondly, a dynamic filtering strategy is proposed to guide the network focus on fundamental semantic parts of each instance rather than backgrounds or distractors during the training stage. Thus, the regression and classification consistency is achieved, so that candidate proposals with high scores usually align with an instance tightly. Since there is no spatial constraint in our method, no hyper-parameters are needed.  

The main contribution of this work lies in the following aspects.
\begin{itemize}
    \item We propose a novel box reorganization method in a unified anchor free detection framework. Especially, a D\&R module is proposed to
    take the boundary prediction as an atomic operation, and then reorganize well-aligned boundaries into boxes in a bottom-up fashion with negligible computation overhead.
    To the best of our knowledge, the idea of breaking boxes into boundaries for training has never been investigated in this task.
    \item We evaluate the semantic inconsistency between center key-points inside an instance and the annotated labels, which helps boost  the convergence of a detection network.
    \item The proposed method DDBNet obtains a state-of-the-art result of 45.5\% in AP. The stable experimental results in all metrics ensure that this method can be effectively extended to typical anchor free detectors.
\end{itemize}

%which depicts it is effective to extend the typical single-stage detector.
%defines a new standard on the challenging COCO dataset with the setting of single-scale and single-model testing.




==> ECCV20-AFOD-final/doc/methods.tex <==

\section{Our Approach}
%In this section, we describe our anchor free model in detail to explain how we take advantage of boundaries instead of boxes to optimize training and enhance prediction results at inference.
In this work, we build DDBNet based on FCOS as a demonstration, which is an advanced anchor-free method. As shown in \Cref{figure: network-structure}, our innovations lie in the box decomposition and recombination (D\&R) module and the semantic consistency module. 

To be specific, the D\&R module reorganizes the predicted boxes by breaking them into boundaries for training which is concatenated behind the regression branch. In the training stage, once bounding box predictions are regressed at each pixel, the D\&R module decomposes each bounding box into four directional boundaries. Then, boundaries of the same kind are ranked by their actual boundary deviations from the ground-truth. Consequently, by recombining ranked boundaries, more accurate box predictions are expected, which are then optimized by the IoU loss \cite{yu2016unitbox}.

As for the semantic consistency module, a new branch of estimating semantic consistency instead of centerness is incorporated into the framework, which is optimized under the supervision of the semantic consistency module. This module exploits an adaptive filtering strategy based on the outputs of the classification and the regression branches. More details about the two modules are provided in the following subsections.

%The classification score and the regression accuracy are considered in our filtering strategy to help the network dynamically focus on the positive pixels inside the target instance without semantic confusion in the training stage. Another 

%and semantic consistency module guarantees the input boxes of D\&R with good quality.

%Specifically, 
% The predicted boundary confidences contribute to the final box reorganization in Box Merging NMS (BM-NMS) at inference. 

%



%In the training stage, once we get a set of predicted boxes by regression of pixels inside an instance, the boundaries of these boxes are decomposed to four sets as left, right, bottom and top set. Each boundary is assigned an original confidence, which is the IoU between the ground-truth and the predicted box where it belongs.
%Then every set of boundaries is ranked by the boundary deviation of the ground-truth instance. As follows, we can recombine the four ranked set to get more accurate boxes. Then the boundary confidence will be updated if this boundary is assigned a new more accurate box. At last, we optimize the boundary prediction under the supervision of IoU loss, which is calculated by the ground-truth and the selected box who makes this boundary more valuable. 
%Additionally, we design an boundary confidence branch for recombination predicted box in the inference stage. Then, BM-NMS algorithm is designed to make full use of the boundary confidence, which achieved the same behavior on train and inference stage. 

%Furthermore, a simple and effective filter strategy is used to dynamically find positive pixels inside the instance. As it is not like centerness branch who has an predefined supervision, a regularization rule is added to make network learning better.


%Feature Pyramid Network (FPN) \cite{OD-CVPR2017-FPN} is used in our approach as the backbone network.
%A pyramid with levels $P_{l}, l=3,4,...,7$ is constructed in this work.
%Note that, each pyramid level has the same channels ($C$), where $C=256$.
%For the level $l$, its resolution is downsampled by $2^{l}$ compared to the input size.
%We refer readers to \cite{OD-CVPR2017-FPN} for more details on backbone settings.
%We add a single deformable convolution layer at the end of regression branch to do the boundary confidences prediction.

% For the regression target assignments, we assign the regression target to the corresponding level depends on the distances between location $i$ to four boundaries $\{d^l_{i}, d^t_{i}, d^r_{i}, d^b_{i}\}$.
% To be more specific, target of location $i$ is assigned to $P_{l}$ if $\max \{d^l_{i}, d^t_{i}, d^r_{i}, d^b_{i}\} \in [r_{l-1}, r_{l}]$, 
% where $r_2 = 0$, $r_7=\infty$ and $r_l=2^{l} \times 8$ for other levels.
% % where $r_2,r_3,r_4,r_5,r_6$ and $r_7$ are set as 0, 64, 128, 256, 512 and $\infty$ respectively.
% % The full network architecture is shown in \Cref{figure: network-structure}.

% Note that two symmetric heads are attached to the FPN for classification and regression respectively.
% Different feature levels share the same heads and no multi branches are needed.
% Besides two heads, a single deformable layer is added for learning boundary confidences. 
%parameter settings
% \subsection{Architecture and Targets Details}
%     \label{subsec:arch-targets-details}


\subsection{Box Decomposition and Recombination}
\label{subsec:box-decom-recom}
% \textbf{Boxes decomposition}. 



Given an instance $I$, every pixel $i$ inside of $I$ regresses a box $p_{i} = \{l_{i}, t_{i}, r_{i}, b_{i}\}$.
The set of predicted boxes is denoted as $B_{I} = \{ p_{0}, p_{1}, \dots, p_{n}\}$, where $l, t, r, b$ denote the left, the top, the right, and the bottom boundaries respectively.
%$i$ is the index of a pixel in $I$.

%Given an instance $I$, pixel $i$ of $I$ in output of regression branch contains the location of predicted box $p_{i} = \{l_{i}, t_{i}, r_{i}, b_{i}\}$ and $B_{I} = \{ p_{0}, p_{1}, ..., p_{n}\}$, where $l, t, r, b$ denote the left, top, right, bottom boundaries and $i$ is the index of pixel of $I$.

\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1.0\linewidth]{D_R-flow} 
    \caption{\textbf{An illustration of the work flow of the D\&R module.}
    For a clear visualization, only three predictions in color are provided for the same ground-truth shown in black.
    % The dashed line with arrow in red is the gradient flow of first term in \Cref{loss: our-iou} and the  dashed line with arrow in black is the gradient flow of second term.
    (a) \textbf{Decomposition:} Break up boxes and assign IoU scores $S_{0}, S_{1}, S_{2}$ of boxes to boundaries as confidence.
    (b) \textbf{Ranking:} The rule how we recombine boundaries to new boxes.
    (c) \textbf{Recombination:} Regroup boundaries as new boxes and assign new IoU scores $S'_{0}, S'_{1}, S'_{2}$ to boundaries as confidence.
    (d) \textbf{Assignment:} Choose the winner confidence as final result.
    The recombined box is shown on the right.}
    \label{figure:D_R-flow}
\end{figure*} 

Normally, an IoU regression loss is expressed as 
\begin{equation}
    \label{loss: origin-iou}
    L_{IoU} = -\frac{1}{N_{pos}}\sum_{I}\sum_{i}^{n} \log(IoU(p_{i}, p^{*}_{I})),
\end{equation} 
where $N_{pos}$ is the number of positive pixels of all instances, $p^{*}_{I}$ is the regression target. Simply, the proposed box decomposition and recombination (D\&R) module is designed to reproduce more accurate $p_{i}$ with the optimization of IoU loss. As shown in \Cref{figure:D_R-flow}, the D\&R module consists of four steps before regularizing the final box predictions based on the IoU regression. More details are described as follows.

\noindent\textbf{Decomposition:} 
A predicted box $p_{i}$ is split into boundaries $l_{i},t_{i},r_{i},b_{i}$ and the IoU $s_{i}$ between $p_{i}$ and $p^{*}_{I}$ is assigned as the confidences of four boundaries, as shown in \Cref{figure:D_R-flow}(a).
For instance $I$, the confidences of boundaries is denoted as a $N \times 4$ matrix $S_{I}$.
Then we group four kinds of boundaries into four sets, which are $left_{I} = \{ l_{0}, l_{1}, ..., l_{n}\}$, $right_{I} = \{ r_{0}, r_{1}, ..., r_{n}\}$, $bottom_{I} = \{ b_{0}, b_{1}, ..., b_{n}\}$, $top_{I} = \{ t_{0}, t_{1}, ..., t_{n}\}$. 

\noindent\textbf{Ranking:} 
Considering the constraint of the IoU loss \cite{yu2016unitbox}, where the larger intersection area of prediction boxes with smaller union area is favored, the optimal box prediction is expected to have the lowest IoU loss. Thus, traversing all the boundaries of the instance $I$ to obtain the optimal box rearrangement $B'_{I}$ is an intuitive choice. However, in this way, the computation complexity is quite expensive, which is $\mathcal{O}(n^4)$. To avoid the heavy computation brought by such brute force method, we apply a simple and efficient ranking strategy.
For each boundary set of instance $I$, the deviations $\delta_{I}^{_l}$, $\delta_{I}^{_r}$, $\delta_{I}^{_b}$, $\delta_{I}^{_t}$ to the targets boundary $p^{*}_{I} = \{ l_{I}, r_{I}, b_{I}, t_{I}\}$ are calculated. Then, boundaries in each set are sorted by the corresponding deviations, as shown in \Cref{figure:D_R-flow}(b). The boundary closer to the ground-truth has the higher rank than the boundary farther. We find that this ranking strategy works well and the ranking noise does not affect the stability of the network training. 

\noindent\textbf{Recombination:} 
As shown in \Cref{figure:D_R-flow}(c), boundaries of four sets with the same rank are recombined as a new box $B'_I = \{ p'_{0}, p'_{1}, \dots, p'_{n}\}$.
Then the IoU $s'_{i}$ between $p'_{i}$ and $p^{*}_{I}$ is assigned as the recombination confidence of four boundaries. 
The confidences of recombination boundaries is expressed as matrix $S'_{I}$ with shape $N \times 4$.

\noindent\textbf{Assignment:} 
Now we get two sets of boundaries scores $S_I$ and $S'_{I}$. As described as \Cref{figure:D_R-flow}(d), the final confidence of each boundary is assigned using the higher score within $S_I$ and $S'_{I}$ instead of totally using $S'_{I}$. This assignment strategy results from the following case, \textit{e.g}.~the recombined low-rank box contains boundaries far away from the ground-truth. Then, the confidences $s'_{i}$ of four boundaries after recombination are much lower than their original one $s_{i}$. The severely drifted confidence scores lead to unstable gradient back-propagation in the training stage. 

Thus, for reliable network training, each boundary is optimized under the supervision of the IoU loss estimated based on the ground-truth and the optimal box with its corresponding better boundary score. Especially, our final regression loss consists of two parts: 
%In this case, the boundary is optimized under the supervision of the IoU between original box and ground-truth, so the gradient of this boundary is updated same as \Cref{loss: origin-iou}.
%Otherwise, the boundary is optimized by the IoU between the ground-truth and the recombined box which make the boundary more valuable.
%Finally, regression loss of our model is expressed as 
\begin{align}
    \label{loss: our-iou}
    \begin{aligned}
        L^{D\&R}_{IoU} = &\frac{1}{N_{pos}}\sum_{I}(\mathds{1}_{\{S'_{I}>S_{I}\}}L_{IoU}(B'_{I}, T_{I}) \\
        &+ \mathds{1}_{\{S_{I} \geqslant S'_{I}\}}L_{IoU}(B_{I}, T_{I})),
    \end{aligned}
\end{align}
where $\mathds{1}_{\{S_{I} \geqslant S'_{I}\}}$ is an indicator function, 
being $1$ if the original score is greater than the recombined one,
vice versa for $\mathds{1}_{\{S'_{I}>S_{I}\}}$.
The gradient of each boundary is selected to update network according to the higher IoU score between the original box and the recombined box.
Compared to the original IoU loss \Cref{loss: origin-iou} where gradients are back-propagated in local receptive fields,
\Cref{loss: our-iou} updates the network in context without extra parameterized computations.
As box in $B'_{I}$ is composed by boundaries from different boxes, 
features are updated in an instance-wise fashion. 
Note that there are no further parameters added in D\&R module. In short, we only change the way how gradient be updated.

\iffalse
In addition, the D\&R module also contains a branch of estimating four boundary confidences which contributes to the final box recombination at the inference stage. 
The branch of estimating boundary confidences is also learnt under the supervision of the boundary scores $\max(S'_I, S_I)$. This branch is concatenated behind the layer of regression tower as shown in \Cref{figure: network-structure}, consisting of a single deformable convolutional layer and a normal convolutional layer for the score prediction. 

The loss function is written as
\begin{align}
    \label{loss: bd-confidence-loss}
    \begin{aligned}
        % L_{bc} = -\frac{1}{N_{pos}}\sum_{I}\mathds{1}_{\{\max(S'_I, S_I) \geq \theta\}} \max(S_I,S'_I)log(S^p_I) \\
        % + (1 - \max(S_I,S'_I)) log(1-S^p_I).
        L_{bc} = &\frac{1}{N_{pos}}\sum_{I}\mathds{1}_{\{\max(S'_I, S_I) \geq \theta\}} CE(S^p_I, \max(S_I,S'_I)),
    \end{aligned}
\end{align}
%where $\mathbf{M} = \mathds{1}_{\{\max(S'_I, S_I) \geq \theta\}}$. 
% $L_{CE}$ denotes the cross entropy loss. 
where $CE$ denotes as cross entropy.
Only boundaries of the high quality whose confidence scores are greater than the threshold $\theta$ are selected for the network learning.  
$S^p_I$ is the set of boundary confidence scores for an instance predicted by the branch. $S_I$ and $S^{'}_I$ denote sets of boundary scores for an instance estimated based on the ground-truth. 
Note that no gradient is back-propagated from this branch to the main branch.
At the inference stage, the boundary confidences predicted in this new branch contribute to the box merging in the BM-NMS, which are further described in \Cref{subsec:bm-nms}. 
\fi
%The boundary scores $\max(S'_I, S_I)$  to each instance $I$ in the training stage, 
%it is natural to take it as confidence of boundaries for merging to optimized boxes at post processing stage, see detail in \Cref{subsec:bm-nms}.
%We add a single deformable convolution layer at the end of regression branch to do the boundary confidences predictions. 
%Note that merged regression features are used as input for this layer and no gradient propagate to the main branch during training. 

% \textbf{How recombine boundaries to boxes.}

\subsection{Semantic Consistency Module}
\label{subsec:reg-cls-consist}
Since the performance of our D\&R module to some extent depends on the box predictions of dense pixels inside an instance, an adaptive filtering method is required to help the network learning focus on positive pixels while rule out negative pixels. Namely, the labeling space of pixels inside an instance is expected to be consistent with their semantics.
%a well defined target space for pixels inside instances is imperative.
Different from previous works \cite{OD-arXiv2019-FoveaBox,OD-ICCV2019-FCOS,OD-CVPR2019-Wang} which pre-define pixels around the center of the bounding box of an instance as the positive, our network evolves to learn the accurate labeling space without extra spatial assumptions in the training stage.

%we focus on the learning procedure to dynamically define the target space with no spatial assumptions.
The formula of semantic consistency is expressed as:
\begin{align}
    \label{semanticeq}
    \begin{aligned}
        \left\{\begin{matrix}
            \overline{C_I}_{\downarrow} \bigcap  \overline{R_I}_{\downarrow}  \gets \text{negative}, 
            % \end{aligned}
            \\
            \\
            % \begin{aligned}
            \overline{C_I}_{\uparrow} \bigcup  \overline{R_I}_{\uparrow}  \gets \text{positive}, \\
            \end{matrix}\right.\\
            c_{i} = \max_{j=0}^{g}(c_{j}) \in C_I,
    \end{aligned}
\end{align}      
% \begin{aligned}
% \end{aligned}
where $R_I$ is the set of IoU scores between the ground-truth and the predicted boxes of pixels inside the instance $I$, 
$\overline{R_I}$ is the mean IoU score of the set $R_I$, $\overline{R_I}_{\downarrow}$ denotes pixels which have lower IoU confidence than the mean IoU $\overline{R_I}$. Inversely, $\overline{R_I}_{\uparrow}$ denotes pixels which have higher IoU confidence than $\overline{R_I}$.
The element $c_{i} \in C_I$ is the maximal classification score among all categories of the i-th pixel, and $g$ denotes the number of categories.
Similarly, $\overline{C_I}_{\downarrow}$ denotes pixels which have lower classification scores than the mean score of $C_{I}$.
Labels of categories are agnostic in this approach so that the predictions of incorrect categories will not be rejected during training.
Finally, as shown in \Cref{figure: consistency-visualize}, the intersection pixels in $\overline{R_I}_{\downarrow}$ and $\overline{C_I}_{\downarrow}$ are assigned negative, while the union pixels in $\overline{R_I}_{\uparrow}$ and $\overline{C_I}_{\uparrow}$ are assigned positive. Meanwhile, if pixels are covered by multiple instances, they prefer to represent the smallest instance.

More to the point, the filtering method determined by \Cref{semanticeq} is able to adaptively control the ratio of positive and negative pixels of instances with different sizes during the training stage, which have a significantly effect on the detection capability of the network. In the experiments, we investigate the performance of different fixed ratio, and then find that the adaptive selection by mean threshold performs best.

%A visualized explanation is shown in \Cref{figure: consistency-visualize}.
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.49\linewidth]{figure/consistency-visualize.pdf} 
    \caption{\textbf{Visualized example of semantic consistency module.}
    The intersection regions of positive regression and positive classification sets are regarded as consistent targets.}  
    %\textit{Best viewed in color.}}
    \label{figure: consistency-visualize}
\end{figure} 

After the labels of pixels are determined autonomously according to the semantic consistency, the inner significance of each positive pixel is considered in the learning process of our network, similarly to the centerness score in FCOS\cite{OD-ICCV2019-FCOS}. Thus, our network is able to emphasize on more important part of an instance and is learnt more effectively. Especially, the inner significance of each pixel is defined as the IoU between the predicted box and the ground-truth. Then, 
%After pixels are dynamically defined as positive and negative samples, as same as centerness branch in FCOS\cite{OD-ICCV2019-FCOS}, we also take the inner significance of positive samples into account to supervise the network to learn more effectively. The inner significance of pixel is assigned as the IoU between prediction box and ground-truth.
an extra branch of estimating the semantic consistency of each pixel is added to the network supervised by the inner significance. 
The loss for semantic consistency is expressed as in \Cref{loss:cls-loss-consistency},
where $r_{i}$ is the output of semantic consistency branch. $IoU(p_{i}, p^*_{I})$ denotes the inner significance of each pixel.
\begin{align}
    \label{loss:cls-loss-consistency}
    % L_{all} = &L_{bc} + L^{D\&R}_{IoU} + \frac{1}{N_{pos}}\sum_{I}\sum_{i}^{N} L_{cls}(c_{i}, c^*_{i}) \\
    % &+ \frac{1}{N_{pos}}\sum_{I}\sum_{i}^{N} L_{con}(r_{i}, IoU(p_{i}, p^*_{i})),
    L_{con} = \frac{1}{N_{pos}}\sum_{I}\sum_{i \in \overline{C_I}_{\uparrow} \bigcup  \overline{R_I}_{\uparrow}} CE(r_{i}, IoU(p_{i}, p^*_{I})).
\end{align}

Generally, the overall training loss is defined as:
\begin{align}
     \label{loss: loss-all}
     \begin{aligned}
         L = L_{cls} + L^{D\&R}_{reg} + L_{con},
     \end{aligned}
 \end{align}
where $L_{cls}$ is the focal loss as in \cite{OD-ICCV2017-RetinaNet}.

%The intersection of two low confidence sets is marked as negative samples, indicating that the same location of pixels in regression and classification branch with scores lower than means are labeled as background consistently.
%As the semantic consistency strategy works at instance level, the model can adaptively control the ratio of positive and negative samples of instances with different sizes during the training.
% On the other hand, the number of positive samples for each instance 

%To verify the advantage of our consistency strategy, we compare our method with heuristic settings applied in previous works \cite{OD-CVPR2019-Zhucc,OD-CVPR2019-Wang,OD-ICCV2019-FCOS}. And we also conduct a constant ratio $c$ setting which replace the $mean$ to explain that the dynamic ratio is important for instances with different sizes.see \Cref{tab:consistency-ablation} in the ablation studies.


% According to the experiments, this regularization t

% Compared with centerness?
% Compared with \cite{OD-ICCV2019-FCOS} using a centerness to down-weight the low-quality boxes appear close the boundaries of instances, 
% the regularization term here is to make sure the training of two branches are consistent.

\iffalse
\subsection{Box Merging Non Maximum Suppression}
Benefiting from the branch of the boundary confidences prediction as mentioned in \Cref{subsec:box-decom-recom},
a modified approach called Box Merging NMS (BM-NMS) is proposed to execute box merging at the inference stage, as detailed in \Cref{alg:r-nms}. 

\label{subsec:bm-nms}
\begin{algorithm}[tbh!]
    \caption{Box Merging Non-maximum suppression}
    \label{alg:r-nms}
    \begin{algorithmic} 
        \State $\mathcal{B}$ and $S^p$ are $N \times 4$ matrices corresponding to initial detection boxes and boundary confidence scores respectively. 
        \State $\mathcal{S}$ presents the classification scores weighted by consistency predictions.
        % \State $\mathcal{R}$ presents the inner significance.
        \State $N_{t}$  is the NMS threshold
        \State $N_{s}$  is the threshold of the boundary confidence 
        \State
        \State \textbf{Input:} $\mathcal{B}=\{b_{1}, ..., b_{N}\}, \mathcal{S}=\{s_{1}, ..., s_{N}\}, S^p=\{s^p_{1}, ..., s^p_{N}\}$.
        \State $\mathcal{D} \gets \{\}$; $\mathcal{T} \gets \mathcal{B}$;
        \While{$\mathcal{T} \neq \O$}
        \State $m \gets arg \max S$; $\mathcal{T} \gets \mathcal{T}-b_{m}$;
        \For{$b_{i}$ in $\mathcal{T}$}
        \If{$IoU(b_{m}, b_{i}) \geqslant N_{t}$}
        \textcolor{blue}{
            \If{$IoU(b_{m}, b_{i}) \geqslant N_{s}$}
            \State $b_{m} \gets \mathds{1}_{\{s^p_{m} \geqslant s^p_{i}\}} b_{m} +  \mathds{1}_{\{s^p_{m} < s^p_{i}\}} b_{i}$;
            \EndIf    
            \textcolor{black}{\Comment{\textrm{Box Merging NMS}} }
        }
        \State $\mathcal{T} \gets \mathcal{T}-b_{i}; \mathcal{S} \gets \mathcal{S}-s_{i}$;
        \EndIf
        \EndFor
        \State $\mathcal{D} \gets \mathcal{D} \bigcup b_{m}$;
        \EndWhile
        \State \Return $\mathcal{D}, \mathcal{S}$;
    \end{algorithmic}
\end{algorithm}

BM-NMS inserts codes of 3 lines to the loop of standard NMS. 
Note that the detection score $s_i$ is the confidence of classification $c_{i}$  multiplied by the inner significance $r_{i}$. 
The merging rule is based on the confidence scores of box $b_{i}$ and $b_{m}$.
% Despite that $b_{i}$ does not have the maximal detection score of the instance, the box $b_{i}$, whose IoU with $b_{m}$ is over threshold $N_{t}$, is suppressed directly in the standard NMS.
The box $b_{i}$, whose IoU with $b_{m}$ is over threshold $N_{t}$, is suppressed directly in the standard NMS.
However, in our algorithm, if its IoU with $b_{m}$ is more than the $N_{s}$,
BM-NMS will check whether there are boundaries of $b_{i}$ better than the boundaries of $b_{m}$ and then recombine better boundaries to $b_{m}$. Simply the detection score of $b_{m}$ stays the same. The procedure of box merging makes NMS much robust with negligible overhead.
\fi




==> ECCV20-AFOD-final/doc/related-works.tex <==
\section{Related Work}
%Brief summary anchor based detection
%The development of deep learning based object detection has attracted much research attention in recent years. Convolutional neural network provide a powerful feature presentation which substantially performance better than the traditional object detection methods with handcrafted features and shallow trainable architectures, such as SIFT \cite{CV-ICCV1999-SIFT} and Histogram of Oriented Gradients (HOG) \cite{CV-CVPR2005-HOG}. Here we focus on the path of deep learning based works. For traditional detection frameworks, we suggest readers to \cite{OD-arXiv2019-Zou} for more details.

%\subsection{Anchor based Object Detectors}
\begin{figure*}[tb!]
    \centering
     \includegraphics[width=0.95\linewidth]{network-structure} 
    \caption{\textbf{An illustration of our network architecture.} Two novel components: the D\&R module and the consistency module are incorporated into a general detection network. The D\&R module carries out box decomposition and recombination in the training stage regularized by the IoU loss and predicts boundary confidences supervised by the boundary deviation. The consistency module selects meaningful pixels whose semantics is consistent with the instance to improve network convergence in the training stage.
    }
    \label{figure: network-structure}
\end{figure*} 

\noindent\textbf{Anchor based Object Detectors.}
In anchor-based detectors, the anchor boxes can be viewed as pre-defined sliding windows or proposals, which are classified as positive or negative samples, with an extra offsets regression to refine the prediction of bounding boxes.
The design of anchor boxes is popularized by two-stage approaches such as Faster R-CNN in its RPNs \cite{OD-TPAMI2017-FasterRCNN}, and single-stage approaches such as SSD \cite{OD-ECCV2016-Liu}, RetinaNet \cite{OD-ICCV2017-RetinaNet}, and YOLO9000 \cite{OD-CVPR2017-YOLO9000}, which has become the convention in a modern detector.
Anchor boxes make the best use of the feature maps of CNNs and avoid repeated feature computation, speeding up the detection process dramatically.
However, anchor boxes result in excessively too many hyper-parameters that are used to describe anchor shapes or to label each anchor box as a positive, ignored or negative sample.
These hyper-parameters have shown a great impact on the final accuracy, and require heuristic tuning.

%Anchor based detection inherits the ideas from traditional sliding window and proposal based detectors  \cite{OD-arXiv2019-Zou}. For example, faster R-CNN \cite{OD-TPAMI2017-FasterRCNN} proposes the Region Proposal Network (RPN), which a shallow fully convolutional network is used to map sliding window anchors to low dimensional features. Works adopted with RPN are summarized as two stage methods.Compared to two-stage approaches, the single stage methods skip the object proposal generation and get prediction on class scores and bounding boxes directly. For example, SSD \cite{OD-ECCV2016-Liu} generates anchors in a dense form and features from different convolutional layers are used to regress and classify the anchor boxes.RetinaNet \cite{OD-ICCV2017-RetinaNet} proposes a focal loss to balance the training contribution between positive and negative anchors.To solve the low recall in YOLOv1 \cite{OD-CVPR2016-YOLO}, YOLOv2 \cite{OD-CVPR2017-YOLO9000} makes use of sliding windows anchors and get more robust recall than precedent version.

\noindent\textbf{Anchor Free Object Detectors.}
Anchor-free detectors directly learn the object existing possibility and the bounding box coordinates without anchor reference.
DenseBox \cite{OD-arXiv2015-DenseBox} is a pioneer work of anchor-free based detectors. While due to the difficulty of handling overlapping situations, it is not suitable for generic object detection.

One successful family of anchor free works \cite{OD-ICCV2019-FCOS,OD-CVPR2019-Zhucc,OD-arXiv2019-FoveaBox,OD-CVPR2019-Wang} adopts the Feature Pyramid network \cite{OD-CVPR2017-FPN} (FPN) as the backbone network and applies direct regression and classification on multi-scale features. These methods treat the bounding box prediction as an atomic task without any further investigations, which bounds the detection accuracy due to the two concerns we discussed in the introduction. 
To avoid the drawback of anchors and refine the box presentations, points based box representation becomes popular recently \cite{OD-ECCV2018-CornerNet,OD-CVPR2019-Zhou,OD-ICCV2019-RepPoints,OD-ICCV2019-CenterNet}. For example, CornerNet \cite{OD-ECCV2018-CornerNet} predicts the heatmap of corners and apply an embedding method to group a pair of corners that belong to the same object. \cite{OD-CVPR2019-Zhou} presents a bottom-up detection framework inspired by the keypoint estimations. Compared to these points based methods, our proposed method has following innovations: 1) Our method focuses on the mid-level boundary representations to achieve a balance between accuracy and robustness of feature modeling; 2) Our method does not need to learn an embedding explicitly while obtaining a reliable boundary grouping to produce the final bounding box predictions.

Furthermore, it is observed that anchor-free methods may produce a number of low-quality predicted bounding boxes at locations that are far from the center of a target object.
In order to suppress these low-quality detections, a novel ``centerness'' branch to predict the deviation of a pixel to the center of its corresponding bounding box is exploited in FCOS \cite{OD-ICCV2019-FCOS}.
This score is then used to down-weight low-quality detected bounding boxes and merge the detection results in NMS. FoveaBox \cite{OD-arXiv2019-FoveaBox} focuses on the object's center motivated by the fovea of human eyes.
It is reasonable to degrade the importance of pixels close to boundaries, but the predefined center field may not cover all cases in the real world, as shown in \Cref{figure:inconsistency-example}.
Thus, we propose an adaptive consistency module to solve the inconsistency issue mentioned above between the semantics of pixels inside an instance and the predefined labels or scores. 

%
%Different from \cite{OD-ECCV2018-CornerNet,OD-CVPR2019-Zhou} where extra supervisions are needed, 
%\cite{OD-ICCV2019-RepPoints} performs the learning in a top-down manner with the deformable convolution \cite{OD-ICCV2017-Dai}.  
%The representation of pseudo boxes are more feature adaptive.

%An intuitive reason to apply these hypotheses is that compared with keypoint-based frameworks \cite{OD-ECCV2018-CornerNet,OD-CVPR2019-Zhou,OD-ICCV2019-CenterNet}, 
%the feature learning space is much larger than predicting points.
%In other words, how to define an appropriate learning targets is important to FPN based anchor free models.
%The consistency module in our framework provide a solution from a new perspective.
%\subsection{Post Processing}

%Non-maximum suppression (NMS) has been the \textit{de-facto} methods for object detection frameworks for many years.The NMS provides an efficient way to identify the unique bounding box for each instance. The greedy NMS algorithm can be summarized into two parts: (1) Clustering. Boxes with IoU over the threshold (0.5 is a convention choice) are considered associating with the same instance.   (2) Pruning. For each cluster, the box with highest score is kept as a confidence prediction contribute to the final result.\cite{OD-ICCV2017-Soft-NMS} decays the detection scores instead of removing which avoid false pruning.\cite{OD-GCPR2016-Hosang,OD-CVPR2017-Hosang} proposed decaying the associated detection scores and learning the NMS directly from data.These methods focus at box level, the BM-NMS in this paper explores in a more fundamental level which break the boxes into boundaries and improve the NMS at side level. A variance voting based NMS is proposed in \cite{OD-CVPR2019-He} which take use of the localization variance learned by KL Loss to merge neighboring bounding boxes. Different from \cite{OD-CVPR2019-He} that merges boxes by coordinate reweighting, BM-NMS merges boxes with boundaries replacement directly.

%\subsection{Receptive Fields Augmentation}CNN based models are inherently limited by its fixed geometric structures. Some works try to solve this problem by designing variant transformable convolution kernels. Atrous convolution \cite{SP-WAVELET1990-Holschneider} which increasing the normal filter's stride is widely used in segmentation tasks \cite{SEGM-ICLR2016-Yu,SEGM-TPAMI2018-Deeplab}. Deformable convolution \cite{OD-ICCV2017-Dai,OD-CVPR2019-Zhuxz} can be seen as a generalized version of atrous convolution and get further improvement on many vision tasks. A recent work on anchor free branch \cite{OD-ICCV2019-RepPoints} inspired by \cite{OD-ICCV2017-Dai,ATTN-NIPS2015-Jaderberg} expanded the usage of adaptive sampling for better object localization.   These approaches solve the issue from a top down manner by spatial sampling.The decomposition and recombination strategy applied in this work try to explore this problem in detection task from a bottom up aspect by changing the backpropagation flow.
% which update the regression features by the . 



% Our work belong to this type.
% \subsection{Detection Consistency}

